Coordinate Descent for Network Linearization

ReLU activations are the main bottleneck in Private Inference that is based on ResNet networks. This is because they incur significant inference latency. Reducing ReLU count is a discrete optimization problem, and there are two common ways to approach it. Most current state-of-the-art methods are based on a smooth approximation that jointly optimizes network accuracy and ReLU budget at once. However, the last hard thresholding step of the optimization usually introduces a large performance loss. We take an alternative approach that works directly in the discrete domain by leveraging Coordinate Descent as our optimization framework. In contrast to previous methods, this yields a sparse solution by design. We demonstrate, through extensive experiments, that our method is State of the Art on common benchmarks.

==> 02_algorithms/onr_small.tex <==
\begin{algorithm}
\caption{\textsc{Reverse Block Coordinate Descent}} 
\label{alg:our_alg_small}
\textbf{Inputs:} A network $f_{\theta, m}(\cdot)$ with parameters $\theta$ and a ReLUs mask $m$, \newline
        a train dataset $\mathcal{D}_{train}$ \newline
        $B$: ReLU budget,  \newline
        $N_{\textrm{random samples}}$ the number of random trails,\newline
        $S [\# \textrm{ReLUs}]$ the number of ReLUs sampled in each trail and\newline
        $t$: accuracy drop tolerance per iteration.
        
    \begin{algorithmic}
        \State The network's ReLU Count is $||m||_0$
        \While {$ReLU > B$}
            \State Do tons of stuff
        \EndWhile
        
    \end{algorithmic}
\end{algorithm}


==> 02_algorithms/optimize_and_reduce.tex <==
\begin{algorithm}[h!]
    \small
    \caption{\textsc{Block Coordinate Descent: Pseudo Code}}
    % \footnotesize
    \begin{algorithmic}[1]
        \State\textbf{Inputs:} A network $f_{\theta, m}(\cdot)$ with parameters $\theta$ and a ReLUs mask $m$, \newline
        a train dataset $\mathcal{D}_{train}$,  \newline
        $B_\textrm{target}[\# \textrm{ReLUs}]$: target ReLU budget,   \newline
        % $B_\textrm{ref}[\# \textrm{ReLUs}]$: reference ReLU budget,   \newline
        $RT$ the number of random tries, \newline
        $DRC [\# \textrm{ReLUs}]$ is the Delta ReLU Count and \newline
        $ADT$ [\%] is the Accuracy Degradation Tolerance. 
        \State We start from a network with $||m||_0 = B_\textrm{ref}[\# \textrm{ReLUs}]$ ReLUs.
        \For{ $t = 1, ..., T = \lceil\frac{B_\textrm{ref} - B_\textrm{target}}{DRC}\rceil$}
            \State $n \leftarrow 0$
            \State $\textrm{found} \leftarrow \textrm{false}$
            \State Initialize a dictionary $d$ which maps binary ReLU maps to their accuracy drops: $d = \{\}$
           \While {$n < \text{RT} \land \textrm{NOT}$$(\textrm{found})$}
                \State Randomly sample $DRC$ ReLUs from the pool of present ReLUs in the mask $m$. We define a mask $m^{\textrm{small}}_n$ such that $||m^{\textrm{small}}_n||_0 = DRC$.
                \State Set $m_{\textrm{hypothesis}} \leftarrow m \odot m^{\textrm{small}}_n$
                \State Evaluate the Accuracy degradation for the current ReLU hypothesis: $\Delta Acc \leftarrow \textrm{Accuracy}(f_{\theta, m}) - \textrm{Accuracy}(f_{\theta, m_{\textrm{hypothesis}}})$
                \If {$\Delta Acc<ADT$}
                    \State found $\leftarrow \textrm{true}$
                    \State $m_{n}^{*} \leftarrow m^{\textrm{small}}_n$
                \EndIf 
                \State Update $d[m^{small}_n] = \Delta Acc $
                \State $n \leftarrow n + 1$
           \EndWhile
           \If {$\textrm{NOT}(\textrm{found})$}
                \State $m_{n}^{*} \leftarrow \argmin _{d.keys()} d.values()$
           \EndIf 
           \State $m \leftarrow m \odot m_{n}^{*}$
           \State Fine-tune the network $f_{\theta, m}(\cdot)$
        \EndFor
    \end{algorithmic}
    \label{alg:our_alg_pseudo_code}
    % \vspace{.825em}
\end{algorithm}


==> figures/00_teaser_figure/00_tikz_teaser_figure.tex <==
%\begin{figure}[!t]
%   \centering
%    \resizebox{0.95\linewidth}{!}{
%    \input{icml2024/tikz/snl_table_cifar100}}
%    \caption{\textbf{CIFAR-100: Accuracy vs ReLU budget: } %Our approach, SNL, achieves the Pareto frontier on ReLU %counts vs.\ test accuracy for CIFAR-100.}
%    \label{fig:C100-pareto-curve}
%\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{figures/02_comparisons/cifar100_results.pdf}
    \caption{\textbf{CIFAR-100: Accuracy vs ReLU budget: } Our approach achieves the Pareto frontier on ReLU counts vs.\ test accuracy for CIFAR-100.}
    \label{fig:C100-pareto-curve}
\end{figure}

==> figures/01_three_datasets_comparison/01_3_datasets.tex <==
% \documentclass{standalone}
% \usepackage{pgfplots}
% \usepackage{pgfplotstable}
% \pgfplotsset{compat=1.16}
%\pgfplotsset{yticklabel style={text width=3em,align=right}}
\usetikzlibrary{pgfplots.groupplots}

\begin{tikzpicture}
    \begin{groupplot}[group style={group size=3 by 1}, cycle list name=color list,
 	xlabel={ReLU Count (in K)},
 	%ylabel={Approximate Accuracy},
 	legend cell align=center,
 	%legend pos=outer north east,
%  	height=6cm,
%  	width=10cm,
 	legend columns=9, 
 	legend style={at={(0.5,1.2)},anchor=north},
 	grid=major,
 	ylabel near ticks,
 	major grid style={dashed},
 	every group plot/.append style={ultra thick},
 	every group plot/.append style={mark size={0pt}}, width=7.5cm]
 	
    \nextgroupplot[ylabel={Test Accuracy}, xmode=log, log basis x=2, 
    /pgf/number format/1000 sep={\,}, log ticks with fixed point,
    title=CIFAR-10, title style={at={(0.5, 0.95)}},]
    
    \addplot+[mark=*,mark size=2pt,blue, thick] 
        plot coordinates {
            (12.9, 88.23)
            (14.9, 88.43) 
            (25.0, 90.88)
            (29.8, 90.92)
            (40.0, 91.68)
            (49.4, 92.27)
            (60.0, 92.63)
            (69.8, 93.02)
            (79.1, 93.16)
            (99.9, 93.50)
            (150.0, 94.26)
            (180.0, 94.78)    % WIde ResNet
            (300, 95.06)
            (400, 95.07)
            (500, 95.21)
            
        };
    % \addlegendentry{ESPN+}
    
    \addplot+[mark=x,mark size=2pt,red, thick, only marks] 
        plot coordinates {
            (36.0 , 88.5)
            (70.0, 90.0)
            (80.0, 90.5)
            (114.0, 92.7)
            (147.0, 93.16)
            (221.48,94.07)
            % (99.8,89.32)
            % (99.9,86.7)
        };
    % \addlegendentry{DeepReduce}
    
    % \addplot+[mark=*,mark size=2pt, brown, thick, only marks] 
    %     plot coordinates {
    %         (25.0, 78.39)
    %         (30.0, 81.0)
    %         (50.0, 83.28)
    %         (60.0, 85.01)
    %         (80.0, 87.21)
    %         (100.0, 88.73)
    %         (150.0, 91.15)
    %     };
    % \addlegendentry{Magnitude}
    
    \addplot+[mark=triangle,mark size=2pt, gray, thick, only marks] 
        plot coordinates {
            (50, 90.0)
            (86, 91.5)
            (100, 92.2)
            (334, 94)
            (500, 94.8)
        };
    % \addlegendentry{CryptoNAS}
    
    \addplot[mark=oplus, mark size=2pt, cyan!80!black, thick, only marks]
        plot coordinates{
            %(37.27, 45.67)
            (152.21, 84.36)
            (110.59, 78.73)
            (211.584, 84.04)
            (301.44, 85.68)
            (337.92, 86.4)
            (442.36, 85.83)
        };
        
    \addplot[mark=otimes, mark size=2pt, violet, thick, only marks]
        plot coordinates{
            (311.7, 93.34)
        };
    % \addlegendentry{LFPC}
    
    \nextgroupplot[xmode=log, log basis x=2, 
    /pgf/number format/1000 sep={\,}, log ticks with fixed point,
    title=CIFAR-100, title style={at={(0.5, 0.95)}},]
    
    \addplot+[mark=*,mark size=2pt,blue, thick] 
        plot coordinates {
            (12.9, 66.53)
            (14.9, 67.17) 
            (25.0, 70.05)
            (29.8, 70.18)
            (40.0, 72.35)
            (49.4, 73.75)
            (60.0, 74.85)
            (69.8, 75.29)
            (79.1, 75.72)
            (99.9, 75.94)  % Wide ResNet
            (120.0, 76.35)
            (150.0, 77.35)
            (180.0, 77.65)
            (248.4, 77.7)
        };
    \addlegendentry{SNL}
    
    \addplot[mark=x,mark size=2pt,red, thick, only marks] 
        plot coordinates {
            (12.3, 64.97)
            (28.7 , 68.68)
            (49.2, 69.50)
            (57.34, 72.68)
            (114.0, 74.72)
            (197.0, 75.51)
            (229.38,76.22)
            % (99.8,89.32)
            % (99.9,86.7)
        };
    \addlegendentry{DeepReduce}
    
    \addplot[mark=pentagon, mark size=2pt, brown, thick, only marks] 
        plot coordinates {
            (25.6, 66.13)
            (30.2, 67.37)
            (41.0, 68.23)
            (51.2, 69.57)
            (71.7, 71.06)
            (102.4, 72.90)
            (230, 74.93)
        };
    \addlegendentry{Sphynx}
    
    % \addplot[mark=*,mark size=2pt, brown, thick, only marks] 
    %     plot coordinates {
    %         (25, 57.89)
    %         (30, 58.31)
    %         (50, 62.6)
    %         (60, 65.50)
    %         (80, 67.60)
    %         (100, 69.82)
    %         (150, 73.07)
    %     };
    % \addlegendentry{Magnitude}
    
    \addplot[mark=triangle,mark size=2pt, gray, thick, only marks] 
        plot coordinates {
            (50, 63.5)
            (86, 66)
            (100, 68.5)
            (334, 76)
            (500, 77)
        };
    \addlegendentry{CryptoNAS}
    
    \addplot[mark=square,mark size=2pt,green, thick, only marks] 
        plot coordinates {
            (110, 67.5)
        };
    \addlegendentry{SAFENet}
    
    \addplot[mark=+,mark size=2pt,yellow!80!black, thick, only marks] 
        plot coordinates {
            (12.9, 56.83)
            (14.9, 56.92)
            (25.0, 60.88)
            (29.8, 62.20)
            (40.0, 61.98)
            (49.4, 63.69)
            (60.0, 64.89)
            (69.8, 64.98)
            (79.1, 65.50)
            (99.9, 66.50)
        };
    \addlegendentry{SNIP}


    \addplot[mark=diamond,mark size=2pt,orange, thick, only marks] 
        plot coordinates {
            (50, 66)
            (180, 67)
            (300, 68)
            % (70,91.56)
            % (80,91.22)
            % (90,91.17)
            % (95,90.93)
            % (99,10.00)
            % (99.5,10.00)
            % (99.8,10.00)
            % (99.9,10.00)
        };
    \addlegendentry{DELPHI}
    
    \addplot[mark=oplus, mark size=2pt, cyan!80!black, thick, only marks]
        plot coordinates{
            % (1179.648,72.13)
            % (875.392,62.31)
            % (808.32, 62.58)
            %(786.186, 61.43)
            (147.9, 52.09)
            (211.84, 54.74)
            (426.638, 60.12)
            %(59.52, 35.91)
            %(37.37, 12.93)
        };
    \addlegendentry{$\ell_1$ Filter Pruning}
    
    \addplot[mark=otimes, mark size=2pt, violet, thick, only marks]
        plot coordinates{
            (311.7, 70.83)
        };
    \addlegendentry{LFPC}
	
    % \addplot+[ultra thick] table[col sep=comma, x=radius, y=accuracy]{Plots/paper_results/CIFAR10/smoothmax_100_25.0.csv};
    % %\addlegendentry{Smooth-max classifier}
	
    % \addplot+[dotted, ultra thick, cyan] table[col sep=comma, x=radius, y=accuracy]{Plots/paper_results/CIFAR10/max_1_25.0.csv};
     %\addlegendentry{Max-smooth Classifier}
     
    %  \node at (axis cs:0.7, 0.65) [anchor = north east] {$\sigma=0.25$};
     
    
     
    %  \addplot+[dashed, ultra thick] table[col sep=comma ,x=radius, y=accuracy]{Plots/paper_results/CIFAR10/salman_base_50.0.csv};
    % \addlegendentry{Base Smooth Classifier}
	
    % \addplot+[ultra thick] table[col sep=comma, x=radius, y=accuracy]{Plots/paper_results/CIFAR10/smoothmax_100_50.0.csv};
    % \addlegendentry{Smooth-max classifier}
	
    % \addplot+[dotted, ultra thick, cyan] table[col sep=comma, x=radius, y=accuracy]{Plots/paper_results/CIFAR10/max_1_50.0.csv};
    %  \addlegendentry{Max-smooth Classifier}
     
    %  \node at (axis cs:1.4, 0.73) [anchor = north east] {$\sigma=0.5$};
     
    \nextgroupplot[xmode=log, log basis x=2, 
    /pgf/number format/1000 sep={\,}, log ticks with fixed point,
    title=Tiny-ImageNet, title style={at={(0.5, 0.95)}},]
    
    \addplot[mark=*,mark size=2pt,blue, thick] 
        plot coordinates {
            (60, 54.24)
            (100, 58.94)
            (200, 63.39)
            (300, 64.04)
            (400, 63.83)
            (500, 64.42)
        };
    % \addlegendentry{ESPN+: ResNet18}
    
 
    \addplot[mark=x,mark size=2pt,red, thick, only marks] 
        plot coordinates {
            % (12.9, 41.95)
            % (24.6, 47.01) 
            % (28.67, 47.55)
            % (49.16, 49.00)
            (57.35, 53.75)
            (98.3, 55.67)
            (114.69, 56.18)
            (200.0, 57.51)
            (230.0, 59.18)
            (400.0, 61.65)
            (459.0, 62.26)
            (917.0, 64.66)
        };
        
    \addplot[mark=pentagon, mark size=2pt, brown, thick, only marks] 
        plot coordinates {
            (102.4, 48.44)
            (204.8, 53.51)
            (286.7, 56.72)
            (491.5, 59.12)
            (614.4, 60.76)
            % (102.4, 72.90)
            % (230, 74.93)
        };
    % \addlegendentry{DeepReduce}
    % \addplot+[dashed, ultra thick] table[col sep=comma ,x=radius, y=accuracy]{Plots/paper_results/CIFAR10/salman_base_100.0.csv};
    % %\addlegendentry{Base Smooth Classifier}
	
    % \addplot+[ultra thick] table[col sep=comma, x=radius, y=accuracy]{Plots/paper_results/CIFAR10/smoothmax_100_100.0.csv};
    % %\addlegendentry{Smooth-max classifier}
	
    % \addplot+[dotted, ultra thick, cyan] table[col sep=comma, x=radius, y=accuracy]{Plots/paper_results/CIFAR10/max_1_100.0.csv};
    %  %\addlegendentry{Max-smooth Classifier}
     
    %  \node at (axis cs:3.0, 0.28) [anchor = north east] {$\sigma=1.00$};
     
    \end{groupplot}
\end{tikzpicture}	


==> figures/03_autorep_hysteresis/autorep_hysteresis.tex <==
% \begin{figure}[t]
%     \centering
%       % \includegraphics[width=0.95\linewidth]{Fig/Forward.pdf}
%       \includegraphics[width=0.8\linewidth]{icml2024/figures/03_autorep_hysteresis/Forward_single_cropped.pdf}
%   \caption{AutoRep's Hysteresis indicator parameter update. }
%     \label{fig:autorep_hysteresis}
% \end{figure}
\begin{figure}
    \centering
    \resizebox{0.98\linewidth}{!}{
    \input{tikz/autoreps_hysteresis}
    }
    \caption{\textbf{AutoRep's Hysteresis which aims at mask values stabilization:} Truncated Gradients~\cite{langford2009sparse} shrink the coefficient to zero by a smaller amount and AutoRep~\cite{peng2023autorep} reduces the possibility of the indicator flip through the suggested hysteresis structure of the indicator value.}
     \label{fig:autorep_hysteresis}
\end{figure}

==> tables/autrep_comparison.tex <==
\begin{table}[]
\centering
\begin{tabular}{|ccc|}
\hline
\multicolumn{3}{|c|}{CIFAR-100}                                                                                                        \\ \hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}ReLU \\ Budget {[}\#K{]}\end{tabular}} & \multicolumn{1}{c|}{AutoRep} & Ours           \\ \hline
\multicolumn{1}{|c|}{6}                                                                & \multicolumn{1}{c|}{71.63}   & \textbf{72.94} \\ \hline
\multicolumn{1}{|c|}{9}                                                                & \multicolumn{1}{c|}{72.39}   & \textbf{73.01} \\ \hline
\multicolumn{1}{|c|}{15}                                                               & \multicolumn{1}{c|}{72.93}       & \textbf{73.7}     \\ \hline
\multicolumn{1}{|c|}{20}                                                               & \multicolumn{1}{c|}{72.8}       & \textbf{73.8}     \\ \hline
\end{tabular}
\caption{\textbf{Our method on top of AutoRep; ResNet18, CIFAR-100: } Our method can be plugged on top of any Selective method. Here we demonstarte the performance gain using our method on top of AutoRep. Our method achieves 72.9\% accuracy with 6K ReLUs, compared with AutoRep which acheives this performance with more than $\times 2$ the number of ReLUs (15K).}
\label{tab:autorep_resnet18_cifar100_comparison}
\end{table}

==> tables/cifar100_ours_vs_autorep_and_snl.tex <==
\begin{table}[b]
\centering
\begin{tabular}{c|cc||cc|}
\cline{2-5}
                                                                                                & \multicolumn{2}{c||}{\textbf{Linearization Methods}}    & \multicolumn{2}{c|}{\textbf{ReLUs $\rightarrow$ Polynomials Methods}} \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}ReLU \\ Budget {[}\#K{]}\end{tabular}}} & \multicolumn{1}{c|}{SNL}   & \textbf{Ours w. Identity} & \multicolumn{1}{c|}{AutoRep}     & \textbf{Ours w. Polynomials}    \\ \hline \hline
\multicolumn{1}{|c|}{6}                                                                         & \multicolumn{1}{c|}{57.65} & \textbf{61.78}            & \multicolumn{1}{c|}{71.69}       & \textbf{72.97}                  \\ \hline
\multicolumn{1}{|c|}{9}                                                                         & \multicolumn{1}{c|}{62.8}  & \textbf{64.8}             & \multicolumn{1}{c|}{71.42}       & \textbf{73.01}                  \\ \hline
\multicolumn{1}{|c|}{12.9}                                                                      & \multicolumn{1}{c|}{66.53} & \textbf{68.24}            & \multicolumn{1}{c|}{74.92}       & ?                               \\ \hline
\multicolumn{1}{|c|}{15}                                                                        & \multicolumn{1}{c|}{67.17} & \textbf{68.74}            & \multicolumn{1}{c|}{73.97}       & ?                               \\ \hline
\multicolumn{1}{|c|}{16.8}                                                                      & \multicolumn{1}{c|}{68.54} & \textbf{69.57}            & \multicolumn{1}{c|}{73.67}       & ?                               \\ \hline
\multicolumn{1}{|c|}{20}                                                                        & \multicolumn{1}{c|}{69.38} & \textbf{69.57}            & \multicolumn{1}{c|}{73.27}       & ?                               \\ \hline
\end{tabular}\caption{\textbf{Test Accuracy[\%] vs. ReLU Budget [\#K] 
for ResNet18 CIFAR-100:} We show that our method outperforms SNL which is the previous SOTA method for Network Linearization, and outperforms AutoRep which is the previous SOTA method for ReLUs replacement with Polynomials for Private Inference.  }
\label{tab:cifar100_snl_vs_our}
\end{table}

==> tables/cifar100_resnet18_comparison.tex <==
\begin{table}
\centering
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{|c|c|c|}
\hline
\textbf{Method}                & \textbf{\# ReLUs {[}K{]}} & \textbf{Test Acc. {[}\%{]}} \\ \hline
\multirow{6}{*}{\textbf{Ours}} & 6                & 61.78              \\ \cline{2-3} 
                      & 9                & 64.8               \\ \cline{2-3} 
                      & 12.9             & 68.24              \\ \cline{2-3} 
                      & 15               & 68.74              \\ \cline{2-3} 
                      & 16.8             & 69.57              \\ \cline{2-3} 
                      & 20               & 69.7               \\ \cline{2-3}
                      & 100              & 76.5               \\ \cline{2-3}
                      & 150              & 77.27              \\ \hline
\multirow{6}{*}{SNL}  & 6                & 57.65              \\ \cline{2-3} 
                      & 9                & 62.8               \\ \cline{2-3} 
                      & 12.9             & 66.53              \\ \cline{2-3} 
                      & 15               & 67.17              \\ \cline{2-3} 
                      & 16.8             & 68.54              \\ \cline{2-3} 
                      & 20               & 69.38              \\ \cline{2-3}
                      & 100              & 75.42              \\ \cline{2-3}
                      & 150              & 76.13              \\ \hline
\multirow{2}{*}{DeepReDuce}  & 28.7      & 68.68              \\ \cline{2-3} 
                      & 49.2             & 69.50              \\ \cline{2-3}
                      & 114              & 74.72              \\ \cline{2-3}
                      & 197              & 75.51              \\ \cline{2-3}
                      & 229.38           & 76.22              \\ \hline
\multirow{3}{*}{CryptoNAS}  & 50      & 63.5              \\ \cline{2-3} 
                      & 86             & 66              \\ \cline{2-3}
                      & 100              & 68.5              \\ \hline
\multirow{6}{*}{SPHYNX} & 25.6           & 66.13              \\ \cline{2-3} 
                      & 30.2             & 67.37              \\ \cline{2-3}
                      & 41.0             & 68.23              \\ \cline{2-3}
                      & 51.2             & 69.57              \\ \cline{2-3}
                      & 71.7             & 71.06              \\ \cline{2-3}
                      & 102.4            & 72.90              \\ \hline
\end{tabular}
}


% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Budget}} & \textbf{SNIP} & \textbf{Sphynx} & \multicolumn{1}{c|}{\textbf{SNL}} & \multicolumn{1}{c|}{\textbf{AutoRep}} & \multicolumn{1}{c|}{\textbf{\textbf{Ours}}} \\ \hline
% 6                                                                                            & -             &                 & 57.65                             & 71.63                                 & \textbf{61.78}                     \\ \hline
% 9                                                                                            & -             &                 & 62.8                              & 71.42                                & \textbf{64.8}                      \\ \hline
% 12.9                                                                                         & 56.83         &                 & 66.53                             & 74.92                                 & \textbf{68.24}                     \\ \hline
% 15                                                                                           & 56.92         &                 & 67.17                             & 73.97                                 & 68.74                              \\ \hline
% 16.8                                                                                         & -             &                 & 68.54                             & 73.67                                & \textbf{69.57}                     \\ \hline
% 20                                                                                           & -             &                 & 69.38                             & 73.27                                & \textbf{69.7}                      \\ \hline
% 25                                                                                           & 60.88         & 66.13           &                                   &                                       &                                    \\ \hline
% 30                                                                                           &               & 67.37           & 70.89                             & 74.45                                   & 70.89                              \\ \hline
% \end{tabular}
\caption{\textbf{CIFAR-100: Accuracy vs ReLU budget: } We evaluate the test classification accuracy versus SOTA}

\label{tab:cifar100_resnet18_comparison}

\end{table}



==> tables/cifar100_resnet18_linearization_and_quadratization.tex <==
\begin{table}
\centering
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{|ccc|}
\hline
\multicolumn{3}{|c|}{\textbf{Linearization}}                                                                                \\ \hline
\multicolumn{1}{|c|}{Method}                                   & \multicolumn{1}{c|}{\# ReLUs {[}K{]}} & Test Acc. {[}\%{]} \\ \hline
\multicolumn{1}{|c|}{\multirow{6}{*}{\textbf{Ours}}}     & \multicolumn{1}{c|}{6}                & 61.78              \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{9}                & 64.8               \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{12.9}             & 68.24              \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{15}               & 68.74              \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{16.8}             & 69.57              \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{20}               & 69.7               \\ \hline
\multicolumn{1}{|c|}{\multirow{6}{*}{SNL}}                     & \multicolumn{1}{c|}{6}                & 57.65              \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{9}                & 62.8               \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{12.9}             & 66.53              \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{15}               & 67.17              \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{16.8}             & 68.54              \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{20}               & 69.38              \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{SNIP}}                    & \multicolumn{1}{c|}{12.9}             & 56.83              \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{15}               & 56.92              \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{25}               & 60.88              \\ \hline
\multicolumn{1}{|c|}{Sphynx}                                   & \multicolumn{1}{c|}{25}               & 66.13              \\ 

\hline \hline
\multicolumn{3}{|c|}{\textbf{ReLUs $\rightarrow$ Polynomials}}                                                                          \\ \hline
\multicolumn{1}{|c|}{Method}                                   & \multicolumn{1}{c|}{\# ReLUs {[}K{]}} & Test Acc. {[}\%{]} \\ \hline
\multicolumn{1}{|c|}{\multirow{6}{*}{\textbf{Ours}}} & \multicolumn{1}{c|}{6}                & 72.97              \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{9}                & 73.01              \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{12.9}             & .                  \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{15}               & ?                  \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{16.8}             & ?                  \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{20}               & ?                  \\ \hline
\multicolumn{1}{|c|}{\multirow{6}{*}{AutoRep}}                 & \multicolumn{1}{c|}{6}                & 71.69              \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{9}                & 71.42              \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{12.9}             & 74.92              \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{15}               & 73.97              \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{16.8}             & 73.67              \\ \cline{2-3} 
\multicolumn{1}{|c|}{}                                         & \multicolumn{1}{c|}{20}               & 73.27              \\ \hline
\end{tabular}
}


% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
% \multicolumn{1}{|c|}{\textbf{Budget}} & \textbf{SNIP} & \textbf{Sphynx} & \multicolumn{1}{c|}{\textbf{SNL}} & \multicolumn{1}{c|}{\textbf{AutoRep}} & \multicolumn{1}{c|}{\textbf{\textbf{Ours}}} \\ \hline
% 6                                                                                            & -             &                 & 57.65                             & 71.63                                 & \textbf{61.78}                     \\ \hline
% 9                                                                                            & -             &                 & 62.8                              & 71.42                                & \textbf{64.8}                      \\ \hline
% 12.9                                                                                         & 56.83         &                 & 66.53                             & 74.92                                 & \textbf{68.24}                     \\ \hline
% 15                                                                                           & 56.92         &                 & 67.17                             & 73.97                                 & 68.74                              \\ \hline
% 16.8                                                                                         & -             &                 & 68.54                             & 73.67                                & \textbf{69.57}                     \\ \hline
% 20                                                                                           & -             &                 & 69.38                             & 73.27                                & \textbf{69.7}                      \\ \hline
% 25                                                                                           & 60.88         & 66.13           &                                   &                                       &                                    \\ \hline
% 30                                                                                           &               & 67.37           & 70.89                             & 74.45                                   & 70.89                              \\ \hline
% \end{tabular}
\caption{\textbf{Linearization and Quadratization: CIFAR-100: Accuracy vs ReLU budget: }\amir{It is this table or the other one~\ref{tab:cifar100_resnet18_comparison} which will appear in the final paper.}}

\label{tab:linearization_and_quadratization_cifar100_resnet18_comparison}

\end{table}



==> tables/cifar100_resnet18_ours_vs_snl.tex <==
\begin{table}[]
\begin{tabular}{|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}ReLU \\ Budget {[}\#K{]}\end{tabular}} & SNL   & \textbf{Ours}  \\ \hline
6                                                                         & 57.65 & \textbf{61.78} \\ \hline
9                                                                         & 62.8  & \textbf{64.8}  \\ \hline
12.9                                                                      & 66.53 & \textbf{68.24} \\ \hline
15                                                                        & 67.17 & \textbf{68.74} \\ \hline
16.8                                                                      & 68.54 & \textbf{69.57} \\ \hline
20                                                                        & 69.38 & \textbf{69.57} \\ \hline
\end{tabular}
\caption{\textbf{Test Accuracy[\%] vs. ReLU Budget [\#K] 
for ResNet18 CIFAR-100:} We show that our method outperforms SNL which is the current SOTA method for Network Linearization.}
\end{table}

==> tables/cifar100_snl_vs_our.tex <==
\begin{table}[h]
\begin{tabular}{|c|c|c|}
\hline

\textbf{\begin{tabular}[c]{@{}c@{}}ReLU \\ Budget {[}\#K{]}\end{tabular}} & SNL   & \textbf{Ours}  \\ \hline
% \multicolumn{1}{|c|}{\textbf{Budget {[}K \#ReLUs{]}}} & \multicolumn{1}{c|}{\textbf{SNL Test Accuracy {[}\%{]}}} & \multicolumn{1}{c|}{\textbf{Our Test Accuracy {[}\%{]}}} \\ \hline

6                                                     & 57.65                                                    & \textbf{61.78}                                           \\ \hline
9                                                     & 62.8                                                     & \textbf{64.8}                                            \\ \hline
15                                                    & 67.17                                                    & \textbf{68.85}                                           \\ \hline
20                                                    & 69.38                                                    & \textbf{69.7}                                            \\ \hline
100                                                   & 75.42                                                    & \textbf{76.5}                                            \\ \hline
150                                                   & 76.13                                                    & \textbf{77.27}                                           \\ \hline
\end{tabular}
% \caption{\textbf{CIFAR-100: Accuracy vs ReLU budget: } We evaluate the test classification accuracy against SOTA}
\caption{\textbf{Test Accuracy[\%] vs. ReLU Budget [\#K] 
for ResNet18 CIFAR-100:} We show that our method outperforms SNL which is the current SOTA method for Network Linearization.}

\label{tab:cifar100_snl_vs_our}
\end{table}

==> tables/cifar10_resnet18_comparison.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|l|l|}
\hline
\textbf{Budget} & \textbf{SNL} & \textbf{Ours} \\ \hline
6                                                  & 84.39                             & \textbf{85.65}                                   \\ \hline
9                                                  & 86.97                             & \textbf{87.49}                                   \\ \hline
14.5                                               & 89.8                              & 89.65                                            \\ \hline

\end{tabular}
\caption{\textbf{CIFAR-10: Accuracy vs ReLU budget:} We evaluate the test classification accuracy for different methods }
\label{tab:cifar10_acc_vs_budget}

\end{table}

==> tables/cifar10_resnet18_linearization_comparison.tex <==
\begin{table}
\centering
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{|c|c|c|}
\hline
\textbf{Method}                & \textbf{\# ReLUs {[}K{]}} & \textbf{Test Acc. {[}\%{]}} \\ \hline
\multirow{5}{*}{\textbf{Ours}} & 6                & 85.65              \\ \cline{2-3} 
                      & 9                & 87.49              \\ \cline{2-3} 
                      & 14.5             & 89.65              \\ \cline{2-3} 
                      & 100              & 93.78              \\ \cline{2-3} 
                      & 150              & 94.94              \\ \hline
\multirow{5}{*}{SNL}  & 6                & 84.39              \\ \cline{2-3} 
                      & 9                & 86.97              \\ \cline{2-3} 
                      & 14.9             & 88.43              \\ \cline{2-3} 
                      & 99.9             & 93.50              \\ \cline{2-3} 
                      & 150              & 94.26              \\ \hline
\multirow{3}{*}{DeepReDuce} & 36         & 88.5              \\ \cline{2-3} 
                      & 114              & 92.7              \\ \cline{2-3} 
                      & 147              & 93.16             \\ \hline
\multirow{3}{*}{CryptoNAS} & 50          & 90.0              \\ \cline{2-3} 
                      & 86               & 91.5              \\ \cline{2-3} 
                      & 100              & 92.2              \\ \cline{2-3}
                      & 334              & 94.0              \\ \hline
\end{tabular}
}
\caption{\textbf{CIFAR-10: Accuracy vs ReLU budget: } We evaluate the test classification accuracy for different methods}

\label{tab:cifar10_resnet18_linearization_comparison}

\end{table}

==> tables/cifar10_snl_vs_our.tex <==
\begin{table}[h]
\begin{tabular}{|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Budget {[}K \#ReLUs{]}}} & \multicolumn{1}{c|}{\textbf{SNL Test Accuracy {[}\%{]}}} & \multicolumn{1}{c|}{\textbf{Our Test Accuracy {[}\%{]}}} \\ \hline
6                                                     & 84.39                                                    & \textbf{85.65}                                           \\ \hline
9                                                     & 86.97                                                    & \textbf{87.49}                                           \\ \hline
14.9                                                  & 88.43                                                    & \textbf{89.65}                                           \\ \hline
100                                                   & 93.50                                                    & \textbf{93.78}                                           \\ \hline
150                                                   & 94.26                                                    & \textbf{94.94}                                           \\ \hline
\end{tabular}
\caption{\textbf{CIFAR-10: Accuracy vs ReLU budget: } We evaluate the test classification accuracy against SOTA}

\label{tab:cifar10_snl_vs_our}
\end{table}

==> tables/reference_budgets.tex <==
\begin{table}[]
\centering
\begin{tabular}{|c|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{Dataset}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Target Budget} \\ $B_{\text{target}}$\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Reference Budget} \\ $B_{\text{ref}}$\end{tabular}} \\ \hline
 \hline
\multirow{2}{*}{CIFAR10}               & $\geq$ 100K                        & 200K                                           \\ \cline{2-3} 
                                       & $<$ 30K                               & 30K                                            \\ \hline \hline
\multirow{2}{*}{CIFAR100}              & $\geq$ 100K                        & 200K                                           \\ \cline{2-3} 
                                       & $<$ 30K                               & 30K                                            \\ \hline \hline
\multirow{4}{*}{TinyImageNet}          & 59.1K                                       & 80K                                            \\ \cline{2-3} 
                                       & 99.6K                                       & 150K                                           \\ \cline{2-3} 
                                       & 150K                                        & 180K                                           \\ \cline{2-3} 
                                       & 200K                                        & 220K                                           \\ \hline
\end{tabular}
\caption{\textbf{What is $B_{\text{ref}}$ for each $B_\text{target}$? } Our algorithm starts from a reference budget $B_{\text{ref}}$ and aims at a target $B_{\text{target}}$. We summarize the respective $B_\textrm{ref}$ budgets for all our experiments.}

\label{tab:reference_budgets}
\end{table}

==> tables/tiny_imagenet_comparison.tex <==
\begin{table}[]
\centering
    \begin{tabular}{|l|l|l|}
    \hline
    \textbf{Budget} & {\textbf{SNL}} & {\textbf{Ours }} \\ \hline
    59.1                                               & 54.24                             & \textbf{56.6}                                    \\ \hline
    \end{tabular}
\caption{\textbf{Tiny-ImageNet: Accuracy vs ReLU budget} We evaluate the test classification accuracy for different methods.}
\label{tab:tiny_imagenet_resnet18_comparison}

\end{table}

==> tables/tiny_imagenet_linearization_comparison.tex <==
\begin{table}
\centering
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{|c|c|c|}
\hline
\textbf{Method}                & \textbf{\# ReLUs {[}K{]}} & \textbf{Test Acc. {[}\%{]}} \\ \hline
\multirow{4}{*}{\textbf{Ours}} & 59.1                & 56.6              \\ \cline{2-3} 
                      & 99.6             & 59.77              \\ \cline{2-3} 
                      & 150              & 62.98              \\ \cline{2-3} 
                      & 200              & 63.97              \\ \hline
\multirow{5}{*}{SNL}  & 59.1             & 54.24              \\ \cline{2-3} 
                      & 99.6             & 58.94              \\ \cline{2-3} 
                      & 150              & 62.12              \\ \cline{2-3} 
                      & 200              & 63.39              \\ \hline
\multirow{3}{*}{DeepReDuce} & 98.3       & 55.67              \\ \cline{2-3} 
                      & 114.69           & 56.18              \\ \cline{2-3} 
                      & 200              & 57.51              \\ \hline
\multirow{2}{*}{SPHYNX} & 102.4          & 48.44              \\ \cline{2-3} 
                      & 204.8            & 53.51              \\ \hline
\end{tabular}
}
\caption{\textbf{TinyImageNet: Accuracy vs ReLU budget: } We evaluate the test classification accuracy for different methods}

\label{tab:tiny_imagenet_resnet18_linearization_comparison}

\end{table}

==> tables/tiny_imagenet_snl_vs_our.tex <==
\begin{table}[h]
\begin{tabular}{|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Budget {[}K \#ReLUs{]}}} & \multicolumn{1}{c|}{\textbf{SNL Test Accuracy {[}\%{]}}} & \multicolumn{1}{c|}{\textbf{Our Test Accuracy {[}\%{]}}} \\ \hline
59.1                                                  & 54.24                                                    & \textbf{56.6}                                            \\ \hline
99.6                                                  & 58.94                                                    & \textbf{59.77}                                           \\ \hline
150                                                   & 62.12                                                    & \textbf{62.98}                                           \\ \hline
200                                                   & 63.39                                                    & \textbf{63.97}                                           \\ \hline
\end{tabular}
\caption{\textbf{Tiny-ImageNet: Accuracy vs ReLU budget} We evaluate the test classification accuracy against SOTA.}
\label{tab:tiny_imagenet_snl_vs_our}
\end{table}
